Near-Optimal Truthful Auction Mechanisms in Secondary Spectrum Markets

In this work, we study spectrum auction problem where each request from secondary users has spatial, temporal, and spectral features. With the requests of secondary users and the reserve price of the primary user, our goal is to design truthful mechanisms that will either maximize the social efficiency or maximize the revenue of the primary user. As the optimal conflict-free spectrum allocation problem is NP-hard, in this work, we design near optimal spectrum allocation mechanisms separately based on the following techniques: derandomized allocation from integer programming formulation, its linear programming (LP) relaxation, and the dual of the LP. We theoretically prove that 1) our near optimal allocation methods are bid monotone, which implys truthful auction mechanisms; and 2) our near optimal allocation methods can achieve a social efficiency or a revenue that is at least $1-\frac{1}{e}$ times of the optimal respectively. At last, we conduct extensive simulations to study the performances (social efficiency, revenue) of the proposed methods, and the simulation results corroborate our theoretical analysis.

==> greedy.tex <==
\subsection{Monotone allocation mechanism}
To ensure the truthfulness of buyers, we further propose a monotone
allocation algorithm, which yields a constant approximation factor, as shown
in \emph{Algorithm \ref{alg:3}}. We use a greedy method to allocate requests in channels more
efficiently.

The basic idea is that we first sort all feasible requests according to
their per-unit prices, and then we scan the requests one by one. For each
request, we either accept it, or reject it. When a new request $r_i $ is
considered according to the scan order, it is immediately accepted if it
can be allocated in one of the feasible channels without conflicting with
any other requests that have been allocated in channels. Otherwise, if the total bid
of requests in a feasible channel $s_j$ that conflict with $r_i $
is smaller than request $r_i$'s bid, we allocate $r_i $ in $s_j $ and delete
all the conflicted requests in $s_j$. In this case, we say that $r_i $
"preempts" these conflicted requests; otherwise, we say $r_i $ is "rejected" by
these conflicting requests. Of course, we can also re-accept the rejected or
preempted requests if there is no confliction after some preemption
happened. The process ends when there are no requests to be scanned.


\begin{algorithm}
\caption{MGCA: Monotone Greedy Channel Allocation}\label{alg:3}
\begin{algorithmic}[1]

\REQUIRE ~
Conflict graph $\mathcal{G}$, location matrix $C$, set of channels $\mathcal{S}$, set $\mathcal{R'}$ sorted in descending order according to $\eta _i$;

\ENSURE ~
channel assignment $X^\ast$ ;


\FOR {$i = 1$ to $n$}
\FOR {$j = 1$ to $m$}
\IF {$c_{i,j} =1$ and $r_i$ can be allocated in $s_j$ without conflicting with any other requests that have been allocated in $s_j$}
\STATE allocate $r_i$ in $s_j$ and set $x_i =1$;
\STATE \text{Break}
\ENDIF
\ENDFOR
\IF {$x_i=0 $}
\FOR {$j$= \text{1 to $m$}}
\IF {the total bid of requests have been allocated in $s_j$ that conflict with $r_i$ is smaller than $\phi_i(b_i)$}
\STATE allocate $r_i$ in $s_j$ and set $x_i =1$;
\STATE \textbf{preempt} all the request conflicting with $r_i$;
\FOR {$k=1$ to $i$}
\IF {$c_{k,j}=1$ and $r_k$ can be allocated in $s_j$ without conflicting with any other requests that have been allocated in $s_j$}
\STATE allocate $r_k$ in $s_j$ and set $x_k=1$;
\ENDIF \ENDFOR
\STATE \text{Break}
\ENDIF \ENDFOR \ENDIF
\ENDFOR \RETURN $X^\ast$;
\end{algorithmic}
\end{algorithm}

Recall that we study two models of the requests, one is the Point model, and the other one
is the Area model. We prove in \emph{Theorem \ref{theo:appfactor32}} that MGCA has a constant approximation ratio in the Point model, or
 in the Area model where $L_i$ is a unit disk.

\begin{theorem}
\label{theo:appfactor32}
MGCA has an approximation ratio at most 32 when it is used to maximize social efficiency or the revenue.
\end{theorem}

\begin{proof}
Let $O_{IP1} $ be the set of requests accepted by the optimal solution of
IP (1), $\mathcal{P}$ be the set of requests accepted by \emph{Algorithm \ref{alg:3}}, $w$ be the
total bids of $O_{IP1} $, ${w}'$ be the total bid of requests that are rejected or
preempted by some requests in $\mathcal{P}$, and ${w}''$ be the total bid of $\mathcal{P}$.
Obviously, if a request in $O_{IP1} $ is not accepted by \emph{Algorithm \ref{alg:3}}, it
must be rejected or preempted by some requests in $\mathcal{P}$. Thus, we can get
that $w\le {w}'+{w}''$. If we define $\rho =w \mathord{\left/ {\vphantom {w
{{w}''}}} \right. \kern-\nulldelimiterspace} {{w}''}$, our goal is to give
the upper bound of $\rho $.


For each request $r_i \in O_{IP1} $, if $r_i $ is rejected or preempted by
$r_j \in \mathcal{P}$, we say that $r_j $ should "account for'' the bid of $r_i $.
In the following, we will analyze of the upper bound of bids that an
arbitrary request $r_j \in \mathcal{P}$ should account for.

For an arbitrary request $r_j \in \mathcal{P}$, the requests it should account
for can be categorized into five types.

Type 1: Request $r_j $ should account for the rejection of $r_i \in O_{IP1}
$, and $a_i <a_j $. Suppose there are $N_1$ requests $\{r_{i1} ,r_{i2,} \ldots ,r_{iN_1} \}$ that belong to type 1.
Since all of these requests belong to $O_{IP1} $ and conflict with each
other in time domain, they must conflict-free in spatial domain. We can take $L_i$ as the centre of the interference
 circle in the Point model, or the centre of the requested unit disk area in the Area model.
  Then, for an arbitrary couple of requests $r_{i1} $ and $r_{i2} $, we can get that
$\angle L_{i1} L_j L_{i2} > \pi \mathord{\left/ {\vphantom {\pi 3}}
\right. \kern-\nulldelimiterspace} 3$. Therefore, we can conclude that
$N_1 \le 5$.

Moreover, if $r_i $ is rejected by more than one request in $\mathcal{P}$, we let
each of these requests only account for part of the bid of $r_i $. Assume
$r_i $ is rejected by requests $\{r_{j1} ,\ldots ,r_{jk}\} $, the bid of
$r_i $ is $\phi _i(b_i) $, and the bid of $r_{jh} $ is $\phi _{jh}(b_{jh}) $. Then, the
bid that request $r_{jh} $ should account for $r_i $ is $\frac{\phi _{jh}(b_{jh})
\phi _i(b_i) }{\sum\nolimits_{h\ = 1}^k {\phi _{jh}(b_{jh}) } }$. According to
our preemption rule in line 6 of \emph{Algorithm \ref{alg:3}}, we can get that $\sum\nolimits_{h\ = 1}^k
{\phi _{jh}(b_{jh}) } \ge \phi _i(b_i) $. So, the inequality $\frac{\phi _{jh}(b_{jh})
\phi _i(b_i) }{\sum\nolimits_{h = 1}^k {\phi _{jh}(b_{jh}) } }\le \phi _i(b_i) $
is tenable. Recall that there are at most 5 requests belong to type 1 for
request $r_j $. Then, we can easily conclude that the total bid of requests that
belong to type 1 is less than 5 times of $\phi _i(b_i) $.

Type 2: $r_j $ should account for the rejection of $r_i \in O_{IP1}
$, and $d_i >d_j $. We can get the same conclusion through the analysis as that of
type 1. Therefore, the total bid of requests that belong to type 2 is less than 5 times of $\phi _i(b_i) $.

Type 3: $r_j $ should account for the rejection of $r_i \in O_{IP1}
$, and $a_i >a_j $, $d_i <d_j $. Since $r_i $ is rejected by $r_j $, and $\eta
_i \le \eta _j $. There are at most 5 requests in the
optimal solution share each time slice allocate to $r_j $. Then, the total bid of requests that belong to type 3 is less than the 5 times of
$\phi _i(b_i) $.

Type 4: $r_j$ should account for the preemption of $r_i \in O_{IP1}
$. Obviously, the total bid of requests that belong to type 4 is less
than $\phi _i(b_i) $ according to our preemption rule.

Type 5: $r_i \in O_{IP1} $ is rejected by the requests that are preempted by
$r_j $. In this case, we say that $r_i $ is rejected by $r_j $ indirectly. The
total bid of requests that belong to type 5 is less than 15 times (the total
bid of type 1, 2 and 3) of the bids of requests that directly reject them. On the
other hand, the total bid of requests directly reject them been preempted by
$r_j $ directly or indirectly, which is less than the bid of $r_j$. Thus,
we can get that the total bid of requests that belong to type 5 is less than 15 times
of the bid of $r_j $.

From the above analysis, $\rho $ can be calculated by
$\rho \le \frac{(1+5+5+5+1+15)\phi _i(b_i) }{\phi _i(b_i) }=32$.
Since the $\rho $ bound holds for all the requests in MGCA,
the approximation factor is 32. \end{proof}

Bid-monotone is critical to the truthfulness of secondary users,
so we will give the proof that MGCA is bid-monotone in the following.

\begin{lemma}
\label{lemma:alg3monotone}
Mechanism MGCA is bid-monotone.
\end{lemma}
\begin{proof}
Suppose request $r_i $ wins the auction with bid $v_i $, and if $r_i $
increases its bid from $v_i $ to $ b_i $, its virtual bid will also
increase from $\phi _i(v_i) $ to $\phi _i(b_i) $. Assume $R(\phi _i(v_i) )$ is
the rank of $r_i $ by bidding $v_i $ in set $\mathcal{R}$. Then, we can get that
$R( \phi _i(b_i) )\ge R(\phi _i(v_i) )$.

Since request $r_i $ wins the auction with bid $v_i $, there is no request
that conflicts with $r_i $ has been accepted by \emph{Algorithm \ref{alg:3}} or all requests that
conflicts with $r_i $ have been preempted by other request. In the first case,
$r_i $ will also win the auction by bidding $b_i $. However, $r_i $ may
be rejected firstly in the latter case if it is scanned before all
requests conflicting with it were preempted by other request. Even in this
situation, $r_i $ will also be reaccepted after all requests conflicting
with it were preempted according to line 10 of \emph{Algorithm \ref{alg:3}}. Therefore, $r_i $ always wins
by bidding $b_i >v_i $, and we finish our proof.
\end{proof}

\subsection{Payment calculation and analysis}

Bid-monotone allocation implies that there is a critical value $b _{i,c} $
for each request such that if request $r_i $ bids higher than $b
_{i,c} $ it always wins, and if $r_i $ bids lower than $b_{i,c} $ it
always loses. It has been proved by Myerson that the auction mechanism is
truthful if we charge each winner its critical value. Therefore, we need to
find the critical value for each winner.

The payment calculation algorithm is depicted as follows. Recall
that $R(\phi _i(b_i) )$ is the rank of $r_i $ by bidding $b_i $ in set $\mathcal{R}$.
We scan all winners one by one, and when request $r_i $ is considered,
we keep the bid of other requests unchanged and let $\phi _{\max }^k $ be
maximal virtual bid of $r_i $ making $R(\phi _i(b_i) )=k$. We first find a
critical bid interval $ [ \phi _{\max }^{k+1} ,\phi _{\max }^k ]$
for $r_i $ such that if $\phi _i(b_i) =\phi _{\max }^k $, $r_i $ wins, and if
$\phi _i(b_i) =\phi _{\max }^{k+1}$, $r_i $ loses. Obviously, $\phi
_{\max }^{k+1} \le \phi _i(b_{i,c}) \le \phi _{\max }^k $, and the rank of
$r_i $ keeps stable when $r_i $ changes its virtual bid in the critical bid
interval $ [ \phi _{\max }^{k+1} ,\phi _{\max }^k ]$. Then we can
compute the critical value of $r_i $ exactly. There are two possible cases
making $r_i $ wins by bidding $\phi _i(b_i) =\phi _{\max }^k $ but loses by
bidding $\phi _i(b_i) =\phi _{\max }^{k+1} $. The first case is that $r_i $
preempts all its conflicting requests by bidding $\phi _i(b_i) =\phi _{\max
}^k $, but be rejected by bidding $\phi _i(b_i) =\phi _{\max }^{k+1} $. In
this case, $\phi _i(b_{i,c}) $ is the virtual bid that is equal to the total bid
of its conflict requests. The latter case is that $r_i $ is preempted by one of
its conflicting requests with virtual bid $\phi _{\max }^{k+1} $ but can't be preempted
with virtual bid $\phi _{\max }^k $. In this case, $\phi _i(b_{i,c}) $ is
the maximum virtual bid that $r_i $ can be preempted.

With the proof that allocation mechanism MGCA is bid-monotone,
we can compute the critical value for each winner. Then we can easily get that

\begin{lemma}
\label{lemma:mbgpvalue}
Mechanism MGCA is value-Truthfulness.
\end{lemma}

\begin{lemma}
\label{lemma:mbgptime}
Mechanism MGCA is time-Truthfulness.
\end{lemma}
\begin{proof}
We assume that each request $r_i $ could only claim a longer time duration
$t_i $ than its actual requirement. Keeping the bidding price stable, if $r_i $
wins by bidding ${t}'_i >t_i $, it always wins by bidding $t_i $. Moreover,
the payment of $r_i $ is time-independent. Therefore, the utility of $r_i $
will not increase after it lies. Unfortunately, $r_i $ may lose by bidding
${t}'_i >t_i $, and its utility may decrease after it lies. This finishes
the proof. \end{proof}

Based on Lemma \ref{lemma:mbgpvalue} and Lemma \ref{lemma:mbgptime}, we get that

\begin{theorem}
Mechanism MGCA is truthful.
\end{theorem}



==> intro.tex <==
The growing demand for limited spectrum resource
poses a great challenge in spectrum allocation and usage \cite{chen2009mining}.
Many organizations, such as the Federal Communications
Commission (FCC), have been attempting to free the under-utilized
license spectrum to meet the demands of secondary users
\cite{jones2008evaluation}. One of the most promising methods is spectrum auction, which provides
sufficient incentive for primary user (\emph{a.k.a seller}) to sublease spectrum to
secondary users (\emph{a.k.a buyers}).

The design of spectrum auction mechanisms are facing two major
challenges. First, spectrum channels can be reused in spatial, temporal, and spectral
domain if the buyers are conflict-free with each other. Thus, how to allocate the requests of buyers in channels optimally is often
an NP-hard problem.
%Second, each channel provided by the license holder has a license area, which means spectrum market is a local market. Then, the %auctions of different local spectrum markets will inevitably influence each other when the license areas of different spectrum %channels have intersections.
Second, truthfulness is regarded as one of the most critical properties, however, it's difficult to
ensure truthfulness in a spectrum auction mechanism with performance guarantee.
%\begin{comment}
%in contrast to
%the physical commodities
%that can be traded all over the world, spectrum is a local
%resource. %For instance, as shown in Figure \ref{fig:auctionmodel},
%Each channel provided by a license holder has a license area, and
%each buyer has a fixed geographical location where
%he hopes to access the channel. It means that spectrum market is a \textbf{local market}, where channels
%can only be sold to the buyers whose locations are within their
%license areas. Second, all buyers
%may only be interested in the usage of channels during some fixed time
%intervals. Thus, buyers who are
%conflict-free with each other can share the same
%channel either in spatial or temporal domain, while physical
%commodities can only be sold to one buyer in the
%traditional auctions. Moreover, the license areas of different spectrum channels
%may have intersections, and buyers' locations can be included in the license areas
%of multiple spectrum channels. Then, the auctions of different local
%spectrum markets will inevitably
%influence each other. Due to these unique characteristics of spectrum,
%designing appropriate
%auction mechanisms for spectrum is more complicated than those traditional goods.
%\end{comment}
%\begin{figure}[!t]
%\centering
%\includegraphics[width=6cm]{auction_model.eps}
%\caption{An instance of the.} \label{fig:auctionmodel}
%\end{figure}

Unfortunately, the challenges mentioned above are seldom fully considered in previous
literatures. Most of the existing studies (\eg ~\cite{xu2010secondary,wangdistrict,fengtahes,zhou2009trust,zhou2008ebay,zhutruthful,jia2009revenue,gopinathanstrategyproof,wu2011small})
take truthfulness and spatial reuse into
consideration, and propose a set of truthful spectrum auction mechanisms. In \cite{zhou2008ebay}, truthfulness is first
designed for spectrum auction, where the spatial reuse is considered. \cite{al2011truthful} and
 \cite{jia2009revenue} focus on maximizing revenue for the auctioneer, and the social efficiency maximization problem is studied in  \cite{gopinathanstrategyproof} and \cite{zhutruthful}. However, all of the literatures introduced above assume that buyers
can share one channel only if they are spatial conflict free with each other. In a more realistic model, the buyers can also share one
channel in temporal domain without causing interference with each other. Therefore, temporal
reuse should also be employed to improve the utilization of spectrums. Following in this direction, temporal
reuse is considered in literatures~\cite{xu2010salsa,dong2012combinatorial,wang2010toda,xu2011tofu,deek2011preempt}.
However, most of the studies that focus on temporal reuse assume that the conflict graph of buyers' geometry locations
is a completed graph for each channel, which means there is no
spatial reuse.
%Dong \etal \cite{dong2012combinatorial} tackle spectrum auction problem by introducing combinatorial auction model which achieves
%time-frequency flexibility. However, the authors do not consider spatial reuse issue in their work \cite{dong2012combinatorial}.
Feng \etal \cite{fengtahes} study the case that spectrum can be reused both in spatial
and temporal domains, and propose a truthful double auction mechanism for spectrum. Nevertheless, performance
guarantee is also neglected in \cite{fengtahes}.
To the best of our knowledge, there is no research on truthful spectrum
auction with performance guarantee, in which spectrums can be reused both on spatial and temporal domains.

%\begin{comment}
%Local market, spatial reuse and temporal reuse are the inherent
%characteristics of practical spectrum
%markets. However, they are seldom fully considered in the previous
%literatures. Most existing spectrum
%auctions treat a spectrum market as a global market~\cite{zhou2008ebay,jia2009revenue,al2011truthful,wu2011small,gopinathanstrategyproof}, \ie buyers cannot access one channel when they
%are outside of this channel's license area.
%Therefore, the assumption of global spectrum market is impractical.
%By following in this direction, some works (\eg \cite{wangdistrict}, \cite{fengtahes}) take the
%local market into consideration, and design a set of truthful
%spectrum auction mechanisms. Most of these works assume that buyers
%can share one channel only if they
%are spatial conflict free with each other. Nevertheless, in a more
%realistic model, the buyers can share one
%channel not only in spatial but also in temporal domain without causing
%interference with each other. Therefore, temporal
%reuse should also be employed to improve utilization of spectrums. Actually, temporal
%reuse is considered in literatures~\cite{xu2010salsa,dong2012combinatorial,wang2010toda,xu2011tofu}.
%Unfortunately, local market and spatial reuse are not studied in depth in these works.
%\end{comment}

To tackle this challenge, we propose a truthful auction framework
for practical spectrum markets in this paper. Maximization of the \emph{\textbf{social efficiency}},
\ie allocating a channel to buyers who \textbf{value} it most, and
maximization of the \emph{\textbf{expected revenue}}, \ie
allocating a channel to buyers who \textbf{pay} it most, both are the
nature goals for spectrum auctions.
Thus, we aim at designing a framework that can flexibly choose the
 optimization goal between social efficiency
 and expected revenue.
Then, we propose a set of channel allocation mechanisms which
can either maximize the social efficiency or the expected revenue, and payment
schemes which ensure the truthfulness of our framework. To the best of
our knowledge, we are the
first to design truthful spectrum auctions while considering spatial and temporal reuse with 
performance guarantee.

The main contributions of this paper are as follows.
\begin{enumerate}
  \item We design a truthful auction framework for practical spectrum markets which can flexibly choose the optimization goal and the channel
allocation and payment mechanism.
  \item We study the case that channels can be reused in both spatial and temporal domains in this paper. However, the
problem of allocating the requests of buyers in channels optimally is an NP-hard problem. To tackle this NP-hardness, we propose a set of
 near-optimal channel allocation mechanisms which
 can either approximate the social efficiency or the expected revenue, but not both simultaneously.
  \item In order to design channel allocation mechanisms that ensure good approximation to the objective functions, we
   %first relax the integer programming (IP) formulation of our channel allocation problem into a linear program (LP) problem, which is solvable in polynomial time. Then, we
    propose a channel allocation mechanism DCA to get
    %transform the optimal fractional solution of this LP problem into
     a feasible solution of the channel allocation problem, whose value is always guaranteed to be at least $1-1/e $ times of the optimal.
 %feasible integer solution of the original IP problem by using a carefully designed randomized rounding procedure that ensures the expected value of the feasible integer solution is at least $1-1/e $ times of the value of the optimal solution. We also propose a derandomization mechanism DCA to get a feasible solution whose value is always guaranteed to be at least $1-1/e $ times of the value of the optimal solution.
  \item We also propose a channel allocation mechanism MDCA with approximation ratio of $1-1/e$, which is a revised version of DCA. However, MDCA is bid monotone, which implies that there is a critical value for each winner. Then, we can easily get that MDCA ensures the truthfulness of buyers.
  \item We further design a channel allocation and payment mechanism CATE to make sure that our spectrum auction mechanism is solvable in polynomial time.
   CATE is also based on the LP relaxation technique, and it gets a channel allocation solution whose expected value is larger than $1-1/e$ times of the optimal.
  \item %Although the mechanisms DCA, MDCA, CATE can be executed
%in polynomial time, their practical running time may still be unacceptable
For large scale spectrum markets,
%To address this possible challenge,
we design a greedy-like first-fit
channel allocation mechanism (MGCA) based on a carefully chosen ordering of
bid requests. We prove that MGCA has a constant approximation
ratio and a critical value based payment rule, which together induce
truthful bidding.
\end{enumerate}

%\begin{comment}
% We design a
%framework for spectrum auction
%which can flexibly choose the optimization goal and the channel
%allocation and payment mechanism.
%Since channels can be reused in both spatial and temporal domain, the
%problem of allocating requests of buyers
%in channels optimally to maximize the social efficiency or the
%expected revenue is NP-hard. It is
%more complex than the problem of matching requests and channels
%optimally only in spatial or
%temporal domain. To tackle this challenge, we first relax the
%integer programming formulation of the channel allocation
%problem into a linear program (LP) problem,
%which is solvable in polynomial time. A fractional solution for
%channel allocation can be
%obtained by solving this LP optimally. Then, we transform this fractional solution into a
%feasible integer solution of the original channel allocation problem
%by using a carefully designed randomized rounding procedure that
%ensures the feasiblility of the solution and good approximation to the
%objective functions. We prove that the \textbf{expected} value of the feasible integer
%solution is at least $1-1/e $ times of the value of the optimal solution. To complete our allocation
%mechanism, we also propose a derandomization algorithm to get a feasible solution whose value
%is always guaranteed to be  at least  $1-1/e $ times of the value of the optimal solution. However, the derandomization
%algorithm should be bid-monotone to ensure the truthfulness of buyers. We cannot prove or disprove
%the bid-monotone property of our first derandomization algorithm. Then,
%we propose a revised derandomization algorithm and prove that this new
%allocation method does satisfy the bid-monotone property.
%It's worthy of attention that our
%allocation mechanisms can either approximate the social efficiency or
%the expected revenue, but not both simultaenously.
%
%Although the channel allocation mechanisms based on LP relaxation technique can be executed
%in polynomial time, its practical running time may still be unacceptable for  large scale spectrum markets.
%To address this possible challenge, we then design a greedy-like first-fit
%channel allocation mechanism based on a carefully chosen ordering of
%bid requests. We prove that our greed allocation method also has a constant approximation
%ratio and a critical value based payment rule, which together induce
%truthful bidding.
%
%Our simulation results show that the performance of the .
%\linote{We have to finish this part}
%\end{comment}

The rest of paper is organized as follows:
Section \ref{sec:prelim} introduces the preliminaries and our design
 objectives.
Section \ref{sec:framework} presents our mechanism design framework
for optimizing the social efficiency or the revenue of the seller.
In Section \ref{sec:lp} and Section \ref{sec:greedy}, we
 propose our allocation algorithm, which is based on derandomization of
 solutions from linear programming, and based on greedy approaches.
Section \ref{sec:simulation} presents our extensive simulations for evaluating the social efficiency, revenue, and spectrum
 utilization efficiency of our methods.
We conclude the paper in Section \ref{sec:conclusion}.

